DIME: Fine-grained Interpretations of Multimodal Models via Disentangled Local Explanations

The ability for a human to understand an Artificial Intelligence (AI) model's decision-making process is critical in enabling stakeholders to visualize model behavior, perform model debugging, promote trust in AI models, and assist in collaborative human-AI decision-making. As a result, the research fields of interpretable and explainable AI have gained traction within AI communities as well as interdisciplinary scientists seeking to apply AI in their subject areas. In this paper, we focus on advancing the state-of-the-art in interpreting multimodal models - a class of machine learning methods that tackle core challenges in representing and capturing interactions between heterogeneous data sources such as images, text, audio, and time-series data. Multimodal models have proliferated numerous real-world applications across healthcare, robotics, multimedia, affective computing, and human-computer interaction. By performing model disentanglement into unimodal contributions (UC) and multimodal interactions (MI), our proposed approach, DIME, enables accurate and fine-grained analysis of multimodal models while maintaining generality across arbitrary modalities, model architectures, and tasks. Through a comprehensive suite of experiments on both synthetic and real-world multimodal tasks, we show that DIME generates accurate disentangled explanations, helps users of multimodal models gain a deeper understanding of model behavior, and presents a step towards debugging and improving these models for real-world deployment. Code for our experiments can be found at https://github.com/lvyiwei1/DIME.

==> tables/examp.tex <==
\begin{table*}[]
\vspace{-3mm}
    \centering
    \footnotesize
    \begin{tabular}{l|l|ll}
    \Xhline{3\arrayrulewidth}
    Category & Count & Example ID & Example Additional Insight \\ \hline
    \begin{tabular}[c]{@{}l@{}}\names\ finds an important multimodal interaction\\ that isn't shown by LIME\end{tabular} & 23 & \begin{tabular}[c]{@{}l@{}}1604\\ (Figure~\ref{fig:examp})\end{tabular} & \begin{tabular}[c]{@{}l@{}}From multimodal interaction image explanation we can see that the model was \\ actually looking at the person's mouth for deciding whether he was happy or not.\end{tabular} \\ \hline
    \begin{tabular}[c]{@{}l@{}}\names\ reveals that the model mostly relies on some specific\\ words in unimodal text contribution to answer question.\end{tabular} & 9 & 704 & \begin{tabular}[c]{@{}l@{}}From disentangled text explanations we can see that unimodal text \\ contribution almost dictated the model's predictions\end{tabular} \\ \hline
    \begin{tabular}[c]{@{}l@{}}\names\ confirms that the model indeed performs the correct \\ multimodal interactions and made prediction based on that,\\ instead of relying on unimodal contributions\end{tabular} & 19 & \begin{tabular}[c]{@{}l@{}}554\\ (Figure~\ref{intro})\end{tabular} & \begin{tabular}[c]{@{}l@{}}From multimodal interactions we can see that the model is indeed able to \\ identify table as the reason for "glass", not the wine glass or bottle \\ (which do supply unimodal support for "glass")\end{tabular} \\ \hline
    Others & 8 & \begin{tabular}[c]{@{}l@{}}1104\\ (Figure~\ref{fig:hydrant})\end{tabular} & \begin{tabular}[c]{@{}l@{}}From multimodal interaction image explanation we can see that the \\ model thought the red part of the hydrant is not part of the hydrant\end{tabular} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    \vspace{1mm}
    \caption{The most common categories of additional insights gained from \names\ over LIME without disentanglement, as well as an example from each category.}
    \label{tab:examp}
    \vspace{-5mm}
\end{table*}

==> tables/mdetr.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|ccc}
        \Xhline{3\arrayrulewidth}
        & Total &  LIME & \names\ \\
        \hline
        Reference & $110$ & $71$ & $73$ \\
        Target  & $97$ & $71$ & $65$ \\
        Total & $207$ & $142$ & $138$ \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    \vspace{1mm}
    \caption{Number of correct Reference/Target objects LIME and \names\ recognizes. As we can see, the two methods can recognize approximately the same amount of correct Reference/Target objects.}
    \label{tab:mdetr}
    \vspace{-3mm}
\end{table}
